Bluetooth Mesh under the Microscope: How much ICN is Inside?

Bluetooth (BT) mesh is a new mode of BT operation for low-energy devices that offers group-based publish-subscribe as a network service with additional caching capabilities. These features resemble concepts of information-centric networking (ICN), and the analogy to ICN has been repeatedly drawn in the BT community. In this paper, we compare BT mesh with ICN both conceptually and in real-world experiments. We contrast both architectures and their design decisions in detail. Experiments are performed on an IoT testbed using NDN/CCNx and BT mesh on constrained RIOT nodes. Our findings indicate significant differences both in concepts and in real-world performance. Supported by new insights, we identify synergies and sketch a design of a BT-ICN that benefits from both worlds.

==> figs/styles.tex <==
\tikzset{
    box/.style = { draw, align=center, rectangle, minimum width=5.00cm, minimum height=0.75cm, font=\sffamily\small, inner sep=0pt, anchor=south west },
    box2/.style = { draw, align=center, rectangle, minimum width=3.4cm, minimum height=0.5cm, font=\sffamily\small, inner sep=0pt, anchor=south west },
    smallboxleft/.style = { box, minimum width=1.5cm, minimum height=0.55cm, text width=1.5cm },
    largeboxright/.style = { box, minimum width=3.45cm, anchor=south east, text width=3.45cm },
    boxshare/.style = { box, minimum width=7.25cm, minimum height=0.5cm, anchor=south east, text width=3.45cm },
    central/.style = { draw, rectangle, fill=Pastel1-A, inner sep=0pt, minimum width=0.75cm, minimum height=0.75cm },
    peripheral/.style = { draw, circle, fill=Pastel1-B, inner sep=0pt, minimum width=0.5cm },
}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

